Review for Handling Missing Data with special missing mechanism

Missing data poses a significant challenge in data science, affecting decision-making processes and outcomes. Understanding what missing data is, how it occurs, and why it is crucial to handle it appropriately is paramount when working with real-world data, especially in tabular data, one of the most commonly used data types in the real world. Three missing mechanisms are defined in the literature: Missing Completely At Random (MCAR), Missing At Random (MAR), and Missing Not At Random (MNAR), each presenting unique challenges in imputation. Most existing work are focused on MCAR that is relatively easy to handle. The special missing mechanisms of MNAR and MAR are less explored and understood. This article reviews existing literature on handling missing values. It compares and contrasts existing methods in terms of their ability to handle different missing mechanisms and data types. It identifies research gap in the existing literature and lays out potential directions for future research in the field. The information in this review will help data analysts and researchers to adopt and promote good practices for handling missing data in real-world problems.

==> sections/0-abstract.tex <==
\begin{abstract}
Missing data poses a significant challenge in data science, affecting decision-making processes and outcomes.
Understanding what missing data is, how it occurs, and why it is crucial to handle it appropriately is
paramount when working with real-world data, especially in tabular data, one of the most commonly used
data types in the real world. Three missing mechanisms are defined in the literature: Missing Completely At Random (MCAR), Missing At Random (MAR), and Missing Not At Random (MNAR), each presenting
unique challenges in imputation. Most existing work are focused on MCAR that is relatively easy to handle.
The special missing mechanisms of MNAR and MAR are less explored and understood. This article reviews existing literature on handling missing values. It compares and contrasts existing methods in terms of their ability to handle different missing mechanisms and data types. It identifies research gap in the existing
literature and lays out potential directions for future research in the field. The information in this review
will help data analysts and researchers to adopt and promote good practices for handling missing data in
real-world problems。

\end{abstract}

==> sections/intro_old.tex <==
\section{Introduction}

% what is missing data and how it occurs?
Missing data refers to the absence of values or information in specific fields or attributes within a dataset. In other words, it occurs when data points are not available or have not been recorded for certain variables or observations. The presence of missing data can arise due to various reasons during data collection, storage, or processing. For instance, in surveys or questionnaires, participants might choose not to answer certain questions, leading to missing data for those specific items. Similarly, in sensor data collected from scientific experiments, missing data can occur if sensors malfunction or fail to record data accurately.\\\\
% Why  handling missing data is important
Handling missing data is of utmost importance in the field of data science, as it presents a significant challenge with the potential to adversely affect decision-making processes and research outcomes. When working with real-world data, dealing with missing values becomes one of the many obstacles encountered. The accuracy and efficiency of data analyse tasks  heavily rely on the quality of the data, making it crucial for data analysts and researchers working with tabular data to effectively address the issue of missing values. Mishandling missing values can lead to biased conclusions, compromised generalizability of findings, and hindered development of robust models. Therefore, it is essential to explore and implement appropriate strategies for handling missing values to ensure accurate and reliable results in data-driven analyses and decision-making processes.
\\\\
The occurrence of missing data can be attributed to various mechanisms, each associated with specific assumptions about the data. Among the commonly recognized mechanisms are Missing Completely At Random (MCAR), Missing At Random (MAR), and Missing Not At Random (MNAR). While each mechanism poses its own challenges, special attention needs to be given to MAR and MNAR, as they represent the most intricate and least understood scenarios without clear assumptions or definitions. These mechanisms, which we refer to as \textbf{Special Missing Mechanisms}, are particularly significant due to their association with sensitive data privacy concerns and the potential provision of hidden information. They introduce additional complexity and challenges in accurately imputing missing values, with significant implications for data analysis and decision-making processes. As such, exploring relevant techniques for managing these diverse missing mechanisms becomes even more imperative.
\\\\
% Current Literature and why this survey is needed. 
The existing literature contains a wealth of studies on missing data imputation, encompassing various methods specifically designed to address missing data with different missing mechanisms. However, a notable disparity exists as most of these studies primarily focus on the most common case of missing completely at random (MCAR), while fewer delve into the more complex cases of missing at random (MAR) and missing not at random (MNAR). Additionally, even for those approaches dealing with special missing mechanisms, a lack of standardized approaches for generating missing data in different experiments hinders our ability to make meaningful comparisons between methods. Consequently, there is a compelling need for a comprehensive survey that accounts for various missing mechanisms, specifically for tabular data—the most prevalent data type.
\\\\
This review aims to bridge this gap by summarizing the mechanisms employed by existing approaches for generating missing data and comparing their methodologies. The survey focuses on imputation techniques and explores their efficacy in handling special missing mechanism. By conducting this thorough investigation, researchers will gain a comprehensive understanding of the suitability and performance of various methods for handling missing data with special missing mechanism, empowering them to make better decisions in addressing missing data challenges in their respective domains.
\\\\
In summary, this review serves as a systematic investigation into the ability of existing methods in handling missing data with special missing mechanisms. The rest of this paper is organized as follows: Section \ref{sec:Background and Preliminary} provides the background on the key features of missing data including missing data, missing pattern and missing mechanism, and the common method of handling missing data. Section \ref{sec:Related Work} discusses the related work and motivation behind the research and identifies the 
research gap. 
Section \ref{sec:Methodology for Missing data Generation} list commonly used missing data generation for Special Missing Mechanism from the literature.
Section \ref{sec:Existing Methods of Handling Missing Data}, introduce on the taxonomy of handling missing data  techniques.   Section \ref{sec:Deletion for Handling Missing Data}, \ref{sec:imputation methods}, \ref{sec:Representation Learning for Handling Missing Data} mainly introduced the methods that dealing with missing data. Section \ref{sec:Evaluation Metrics} reviews the evaluation metrics used to measure their performance. Furthermore, Section \ref{sec:Limitations} presents challenges and future direction of the works.

==> tikz/mech_compare.tex <==
\begin{figure}[!h]
    \centering

\begin{tikzpicture}[yscale=0.7, xscale = 0.7]
    \begin{axis}[
        width=0.9*\textwidth,
        x tick label style={/pgf/number format/1000 sep=},[
    %title={Temperature dependence of CuSO\(_4\cdot\)5H\(_2\)O solubility},
    %xlabel={Temperature [\textcelsius]},
    ylabel={Year},
    xmin=2000, xmax=2022,
    ymin=0, ymax=15,
    xtick = {2000,2001,2002,2003,2004,2005,2006,2007,2008,2009,2010,2011,2012,2013,2014,2015,2016,2017,2018,2019,2020,2021,2022},
    ytick={0,5,10,15},
    xticklabel style={rotate=45, anchor=north east},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
]


    % \begin{axis}[
    %     width=1*\textwidth,
    %     x tick label style={/pgf/number format/1000 sep=},
    %     % title={Neural Network Based Imputation Method by Year},
    %     %ylabel=Population,
    %     enlargelimits=0.05,
    %     % Set minimum y value to 0
    %     ymax=50, % Set maximum y value to an integer value
    %     legend pos=north west, % Change legend location
    %     ybar,
    %     bar width=4pt,
    %     xtick={2000,2001,2002,2003,2004,2005,2006,2007,2008,2009,2010,2011,2012,2013,2014,2015,2016,2017,2018,2019,2020,2021,2022,2023},
    %     %ytick={0, 1, 2, 3, 4,5},
    %     xticklabel style={rotate=45, anchor=north east}
    %     ]

\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
%(2023,	8)
(2022,	12)
(2021,	12)
(2020,	4)
(2019,	4)
(2018,	5)
(2017,	6)
(2016,	2)
(2015,	3)
(2013,	5)
(2012,	5)
(2011,	1)
(2010,	1)
(2008,	2)
(2004,	1)
(2003,	1)
(2000,	0)
    };
    \legend{\# Articles occurs in Scopus Database}
    
\end{axis}
\end{tikzpicture}

    \caption{Keyword search from Scopus database for Imputation Method Involving Special Missing Mechanism by Year\\ Keywords: MAR, MCAR, }
    \label{fig:Imputation Method Involving Special Missing Mechanism by Year}

\end{figure}
